DeiT III: Revenge of the ViT

A Vision Transformer (ViT) is a simple neural architecture amenable to serve several computer vision tasks. It has limited built-in architectural priors, in contrast to more recent architectures that incorporate priors either about the input data or of specific tasks. Recent works show that ViTs benefit from self-supervised pre-training, in particular BerT-like pre-training like BeiT. In this paper, we revisit the supervised training of ViTs. Our procedure builds upon and simplifies a recipe introduced for training ResNet-50. It includes a new simple data-augmentation procedure with only 3 augmentations, closer to the practice in self-supervised learning. Our evaluations on Image classification (ImageNet-1k with and without pre-training on ImageNet-21k), transfer learning and semantic segmentation show that our procedure outperforms by a large margin previous fully supervised training recipes for ViT. It also reveals that the performance of our ViT trained with supervision is comparable to that of more recent architectures. Our results could serve as better baselines for recent self-supervised approaches demonstrated on ViT.

==> figure_rrc.tex <==
\begin{figure}
    \centering
    \begin{tabular}{cccccc}
         \multicolumn{2}{c}{\includegraphics[width = 0.3\linewidth]{data_aug/RRC/org_pexels-charl-durand-6476604.jpg}}& 
         \multicolumn{2}{c}{\includegraphics[width = 0.3\linewidth]{data_aug/RRC/org_pexels-gabriela-palai-507410.jpg}}&
         \multicolumn{2}{c}{\includegraphics[width = 0.25\linewidth]{data_aug/RRC/org_pexels-jess-vide-4319846.jpg}} \\
         SRC & RRC & SRC & RRC &  SRC & RRC\\
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/crp_0_pexels-charl-durand-6476604.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/rrc_0_pexels-charl-durand-6476604.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/crp_0_pexels-gabriela-palai-507410.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/rrc_0_pexels-gabriela-palai-507410.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/crp_0_pexels-jess-vide-4319846.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/rrc_0_pexels-jess-vide-4319846.jpg} \\         
         
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/crp_1_pexels-charl-durand-6476604.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/rrc_1_pexels-charl-durand-6476604.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/crp_1_pexels-gabriela-palai-507410.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/rrc_1_pexels-gabriela-palai-507410.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/crp_1_pexels-jess-vide-4319846.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/rrc_1_pexels-jess-vide-4319846.jpg} \\   
         
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/crp_2_pexels-charl-durand-6476604.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/rrc_2_pexels-charl-durand-6476604.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/crp_2_pexels-gabriela-palai-507410.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/rrc_2_pexels-gabriela-palai-507410.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/crp_2_pexels-jess-vide-4319846.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/rrc_2_pexels-jess-vide-4319846.jpg} \\  
         
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/crp_3_pexels-charl-durand-6476604.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/rrc_3_pexels-charl-durand-6476604.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/crp_3_pexels-gabriela-palai-507410.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/rrc_3_pexels-gabriela-palai-507410.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/crp_3_pexels-jess-vide-4319846.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/rrc_3_pexels-jess-vide-4319846.jpg} \\        
        
        \includegraphics[width = 0.14\linewidth]{data_aug/RRC/crp_4_pexels-charl-durand-6476604.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/rrc_4_pexels-charl-durand-6476604.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/crp_4_pexels-gabriela-palai-507410.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/rrc_4_pexels-gabriela-palai-507410.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/crp_4_pexels-jess-vide-4319846.jpg} &
         \includegraphics[width = 0.14\linewidth]{data_aug/RRC/rrc_4_pexels-jess-vide-4319846.jpg} \\    
    \end{tabular}
    \caption{Illustration of Random Resized Crop (RRC) and Simple Random Crop (SRC). The usual RRC is a more aggressive data-augmentation than SRC: It has a more important regularization effect and avoids overfitting by giving more variability to the images. At the same time it introduces a discrepancy of scale and possibly labeling error, for instance when the object is not in the cropped region. On Imagenet1k this regularization is usually regarded as beneficial. However our experiments show that it is detrimental on Imagenet22k, which is less prone to overfitting. 
    \label{fig:fig_rrc}}
\end{figure}

==> figure_rrc_2.tex <==
\begin{figure}
    \centering
    \begin{tabular}{cc}
         RRC &  SRC \\
        \includegraphics[width =0.48\linewidth]{data_aug/roc_fig/rrc_crop.png}& \includegraphics[width =0.48\linewidth]{data_aug/roc_fig/random_crop.png}\\
    \end{tabular}
    \caption{We compare the position of the crops for Random Resized Crop (RRC) and Simple Random Crop (SRC)}. 
    \label{fig:rrc_bbox}
\end{figure}
